Spectral Sparsification for Communication-Efficient Collaborative Rotation and Translation Estimation

We propose fast and communication-efficient optimization algorithms for multi-robot rotation averaging and translation estimation problems that arise from collaborative simultaneous localization and mapping (SLAM), structure-from-motion (SfM), and camera network localization applications. Our methods are based on theoretical relations between the Hessians of the underlying Riemannian optimization problems and the Laplacians of suitably weighted graphs. We leverage these results to design a collaborative solver in which robots coordinate with a central server to perform approximate second-order optimization, by solving a Laplacian system at each iteration. Crucially, our algorithms permit robots to employ spectral sparsification to sparsify intermediate dense matrices before communication, and hence provide a mechanism to trade off accuracy with communication efficiency with provable guarantees. We perform rigorous theoretical analysis of our methods and prove that they enjoy (local) linear rate of convergence. Furthermore, we show that our methods can be combined with graduated non-convexity to achieve outlier-robust estimation. Extensive experiments on real-world SLAM and SfM scenarios demonstrate the superior convergence rate and communication efficiency of our methods.

==> include/custommacros.tex <==
\newcommand{\CommGraph}{\mathcal{G}}
\newcommand{\CommLinks}{\mathcal{E}}
\newcommand{\CommLaplacian}{L}

==> tables/sfm_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

\begin{table*}[t]
	\centering
	\renewcommand{\arraystretch}{1.1}
	\caption{{Robust rotation averaging on real-world SfM datasets. 
			Each dataset is divided to simulate 5 robots.
			$|\Vcal|$ and $|\Ecal|$ denote the total number of rotation variables and measurements, respectively.
			Using the reference solution, 
                we quantify the difficulty of each dataset 
                by computing the percentage of high-quality inlier measurements (measurement error $< 5$~deg)
			and gross outliers (measurement error $> 45$~deg).
			For the proposed method, we show the sparsity achieved by sparsification (lower is better) and total communication.
		}}
	\label{tab:sfm}
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|l|r|r|rrr|rrr|r|rr|}
			\hline
			\multirow{2}{*}{DATASETS} &
			\multicolumn{1}{c|}{\multirow{2}{*}{$|\Vcal|$}} &
			\multicolumn{1}{c|}{\multirow{2}{*}{$|\Ecal|$}} &
			\multicolumn{3}{c|}{Measurement Quality (\%)} &
			\multicolumn{3}{c|}{Mean Error (deg)} &
			\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Achieved \\ sparsity (\%)\end{tabular}}} &
			\multicolumn{2}{c|}{Communication (MB)} \\ \cline{4-9} \cline{11-12} 
			&
			\multicolumn{1}{c|}{} &
			\multicolumn{1}{c|}{} &
			\multicolumn{1}{c|}{Inlier} &
			\multicolumn{1}{c|}{Outlier} &
			\multicolumn{1}{c|}{Other} &
			\multicolumn{1}{c|}{Initial} &
			\multicolumn{1}{c|}{No GNC} &
			\multicolumn{1}{c|}{With GNC} &
			\multicolumn{1}{c|}{} &
			\multicolumn{1}{c|}{Upload} &
			\multicolumn{1}{c|}{Download} \\ \hline
			Montreal Notre Dame &
			468 &
			49705 &
			\multicolumn{1}{r|}{81} &
			\multicolumn{1}{r|}{4} &
			15 &
			\multicolumn{1}{r|}{4.2} &
			\multicolumn{1}{r|}{3.3} &
			1.1 &
			55.1 &
			\multicolumn{1}{r|}{2.09} &
			1.21 \\ \hline
			Ellis Island &
			241 &
			19507 &
			\multicolumn{1}{r|}{63} &
			\multicolumn{1}{r|}{1} &
			26 &
			\multicolumn{1}{r|}{7.0} &
			\multicolumn{1}{r|}{5.6} &
			2.3 &
			66.0 &
			\multicolumn{1}{r|}{0.95} &
			0.57 \\ \hline
			NYC Library &
			355 &
			17579 &
			\multicolumn{1}{r|}{61} &
			\multicolumn{1}{r|}{6} &
			33 &
			\multicolumn{1}{r|}{4.3} &
			\multicolumn{1}{r|}{4.3} &
			2.3 &
			75.8 &
			\multicolumn{1}{r|}{1.24} &
			0.83 \\ \hline
			Notre Dame &
			553 &
			97764 &
			\multicolumn{1}{r|}{70} &
			\multicolumn{1}{r|}{9} &
			21 &
			\multicolumn{1}{r|}{3.5} &
			\multicolumn{1}{r|}{4.5} &
			2.4 &
			41.8 &
			\multicolumn{1}{r|}{2.85} &
			1.54 \\ \hline
			Roman Forum &
			1099 &
			53989 &
			\multicolumn{1}{r|}{74} &
			\multicolumn{1}{r|}{3} &
			23 &
			\multicolumn{1}{r|}{16.5} &
			\multicolumn{1}{r|}{5.1} &
			2.5 &
			68.1 &
			\multicolumn{1}{r|}{4.43} &
			2.73 \\ \hline
			Alamo &
			606 &
			87725 &
			\multicolumn{1}{r|}{74} &
			\multicolumn{1}{r|}{3} &
			23 &
			\multicolumn{1}{r|}{8.0} &
			\multicolumn{1}{r|}{4.5} &
			2.9 &
			44.7 &
			\multicolumn{1}{r|}{2.62} &
			1.39 \\ \hline
			Madrid Metropolis &
			379 &
			18811 &
			\multicolumn{1}{r|}{47} &
			\multicolumn{1}{r|}{20} &
			33 &
			\multicolumn{1}{r|}{7.7} &
			\multicolumn{1}{r|}{8.0} &
			3.4 &
			70.3 &
			\multicolumn{1}{r|}{1.48} &
			1.08 \\ \hline
			Yorkminster &
			448 &
			24416 &
			\multicolumn{1}{r|}{73} &
			\multicolumn{1}{r|}{5} &
			22 &
			\multicolumn{1}{r|}{8.3} &
			\multicolumn{1}{r|}{4.5} &
			3.4 &
			76.5 &
			\multicolumn{1}{r|}{1.69} &
			1.1 \\ \hline
			Tower of London &
			493 &
			19798 &
			\multicolumn{1}{r|}{76} &
			\multicolumn{1}{r|}{3} &
			21 &
			\multicolumn{1}{r|}{7.4} &
			\multicolumn{1}{r|}{4.7} &
			3.5 &
			75.3 &
			\multicolumn{1}{r|}{2.00} &
			1.35 \\ \hline
			Trafalgar &
			5433 &
			680012 &
			\multicolumn{1}{r|}{63} &
			\multicolumn{1}{r|}{7} &
			30 &
			\multicolumn{1}{r|}{20.0} &
			\multicolumn{1}{r|}{6.4} &
			3.5 &
			40.7 &
			\multicolumn{1}{r|}{35.89} &
			24.97 \\ \hline
			Piazza del Popolo &
			343 &
			22342 &
			\multicolumn{1}{r|}{82} &
			\multicolumn{1}{r|}{4} &
			14 &
			\multicolumn{1}{r|}{5.4} &
			\multicolumn{1}{r|}{7.8} &
			3.6 &
			70.0 &
			\multicolumn{1}{r|}{1.29} &
			0.8 \\ \hline
			Piccadilly &
			2436 &
			254175 &
			\multicolumn{1}{r|}{58} &
			\multicolumn{1}{r|}{10} &
			32 &
			\multicolumn{1}{r|}{13.9} &
			\multicolumn{1}{r|}{14.6} &
			4.9 &
			53.1 &
			\multicolumn{1}{r|}{14.23} &
			9.79 \\ \hline
			Union Square &
			930 &
			25561 &
			\multicolumn{1}{r|}{57} &
			\multicolumn{1}{r|}{6} &
			37 &
			\multicolumn{1}{r|}{11.9} &
			\multicolumn{1}{r|}{10.9} &
			6.0 &
			82.1 &
			\multicolumn{1}{r|}{4.15} &
			3.37 \\ \hline
			Vienna Cathedral &
			900 &
			96546 &
			\multicolumn{1}{r|}{70} &
			\multicolumn{1}{r|}{6} &
			24 &
			\multicolumn{1}{r|}{13.9} &
			\multicolumn{1}{r|}{9.6} &
			8.9 &
			51.9 &
			\multicolumn{1}{r|}{4.62} &
			3.13 \\ \hline
			Gendarmenmarkt &
			723 &
			42980 &
			\multicolumn{1}{r|}{36} &
			\multicolumn{1}{r|}{27} &
			37 &
			\multicolumn{1}{r|}{45.0} &
			\multicolumn{1}{r|}{40.8} &
			38.1 &
			63.8 &
			\multicolumn{1}{r|}{4.13} &
			3.03 \\ \hline
		\end{tabular}%
	}
\end{table*}
